Learning to Caricature via Semantic Shape Transform

Caricature is an artistic drawing created to abstract or exaggerate facial features of a person. Rendering visually pleasing caricatures is a difficult task that requires professional skills, and thus it is of great interest to design a method to automatically generate such drawings. To deal with large shape changes, we propose an algorithm based on a semantic shape transform to produce diverse and plausible shape exaggerations. Specifically, we predict pixel-wise semantic correspondences and perform image warping on the input photo to achieve dense shape transformation. We show that the proposed framework is able to render visually pleasing shape exaggerations while maintaining their facial structures. In addition, our model allows users to manipulate the shape via the semantic map. We demonstrate the effectiveness of our approach on a large photograph-caricature benchmark dataset with comparisons to the state-of-the-art methods.

==> conclusions.tex <==

\section{Conclusions}

In this paper, we propose a semantic dense shape transformation algorithm for learning to caricature.
%
%In order to perform the shape and style domain shifts, the input photo is first fed into a shape transformation network, followed by a style transfer process.
%
%For shape transformation, we utilize a face parsing map to densely predict warping parameters, such that the shape exaggerations are effectively transferred while the facial structure is still maintained.
Specifically, we utilize a face parsing map to densely predict warping parameters, such that the shape exaggerations are effectively transferred while the facial structure is still maintained.
%
Visual comparisons and user studies demonstrate that the proposed algorithm is able to generate high-quality caricatures against state-of-the-art methods.
%
In addition, we show that the learned embedding space of semantic parsing map allows us to directly manipulate the parsing map and generate shape changes according to the user preference.
% Although in this work we only evaluate our approach on caricature generation, it is not limited to the specific task of image translation.
% %
% The proposed method can be extended to nume
rous challenging image translation problems which require complex shape deformation.


% DO NOT INCLUDE ACKNOWLEDGMENTS IN AN ANONYMOUS SUBMISSION TO SIGGRAPH 2019
%\begin{acks}
%
%The authors would like to thank Dr. Maura Turolla of Telecom
%Italia for providing specifications about the application scenario.
%
%The work is supported by the \grantsponsor{GS501100001809}{National
%  Natural Science Foundation of
%  China}{http://dx.doi.org/10.13039/501100001809} under Grant
%No.:~\grantnum{GS501100001809}{61273304\_a}
%and~\grantnum[http://www.nnsf.cn/youngscientists]{GS501100001809}{Young
%  Scientists' Support Program}.
%
%
%\end{acks}


==> introduction_tmp.tex <==

\section{Conclusions}
%
Caricature is a rendered image by abstracting or exaggerating certain facial features (e.g., contour, eyes, ear, eyebrows, mouth, and nose) of a person to achieve humorous or sarcastic effects (Fig.~\ref{fig:teaser}).
%
Caricatures are widely used to depict celebrities or politicians for certain purposes in all kinds of media.
%
However, generating visually pleasing caricatures with proper shape distortions usually requires professional artistic skills with creative imaginations, which is a challenging task for common users.
%
Therefore, it is of great interest if caricatures can be generated from normal photos effectively or in a way that users are allowed to flexibly manipulate the output with user controls.
%

One crucial factor to generate a desirable caricature is to distort facial components properly, i.e., to render personal traits with certain exaggerations. 
%
Numerous efforts have been made to perform shape exaggeration by computing warping parameters between photos and caricatures from user-defined shapes~\citep{akleman2000making} or hand-crafted rules~\citep{brennan2007caricature,liao2004automatic}.
%
However, such methods may have limitations on generating diverse and visually pleasing results due to inaccurate shape transformations. 
%
Recently, image-to-image translation~\citep{isola2017image,zhu2017unpaired,DRIT} and neural style transfer~\citep{gatys2016image,johnson2016perceptual,li2017diversified} algorithms have been developed,
%
but most techniques can be applied to two domains with local texture variations, not for scenarios where large shape discrepancy exists.
%

In this work, we aim to create shape exaggerations on standard photos with shape transformations similar to those drawn by artists.
%
Meanwhile, a rendered caricature should still maintain the facial structure and personal traits.
%
Different from existing methods that only consider facial landmarks or sparse points \citep{cao2018carigans,shi2019warpgan}, we use a semantic face parsing map, i.e., a dense pixel-wise parsing map, to guide the shape transformation process.
%
As such, this can provide more accurate mapping for facial details, e.g., shapes of eyebrows, noses, and face contours, to name a few.
%
Specifically, given an unpaired caricature with a normal photo, we leverage the cycle consistency strategy and an encoder-decoder architecture to model the shape transformation.
%
Nevertheless, operating this learning process in the image domain may involve noise from unnecessary information in pixels.
%
Instead, we learn the model directly on the face parsing map, which is the shape transformation of interest.
%
To learn effective shape transformation, we design a spatial transformer network (STN) to allow larger and flexible shape changes, while a few loss functions are introduced to better maintain facial structures.


To evaluate the proposed framework, we conduct experiments on the photo-caricature benchmark dataset \citep{HuoBMVC2018WebCaricature}.
%
We perform extensive ablation studies to validate each component of the proposed shape transformation algorithm.
%
We conduct qualitative and quantitative experiments with user studies to demonstrate that the proposed approach performs favorably against existing image-to-image translation and caricature generation methods.
%
Furthermore, our model allows users to select the desired caricature semantic shape, with the flexibility to manipulate the parsing map to generate preferred shapes and diverse caricatures.
%


